Mitigation of Backgrounds from Cosmogenic $^{137}$Xe in Xenon Gas Experiments using $^{3}$He Neutron Capture

\Xe{136} is used as the target medium for many experiments searching for \bbnonu. Despite underground operation, cosmic muons that reach the laboratory can produce spallation neutrons causing activation of detector materials. A potential background that is difficult to veto using muon tagging comes in the form of \Xe{137} created by the capture of neutrons on \Xe{136}. This isotope decays via beta decay with a half-life of 3.8 minutes and a \Qb\ of $\sim$4.16 MeV. This work proposes and explores the concept of adding a small percentage of \He{3} to xenon as a means to capture thermal neutrons and reduce the number of activations in the detector volume. When using this technique we find the contamination from \Xe{137} activation can be reduced to negligible levels in tonne and multi-tonne scale high pressure gas xenon neutrinoless double beta decay experiments running at any depth in an underground laboratory.

==> Helium3 (2)/src/Authors.tex <==
\collaboration{The NEXT Collaboration}
%
\author[3,a]{L.~Rogers,\note[a]{Corresponding author.}}
%
\author[3]{B.J.P.~Jones,}
%
\author[3]{A.~Laing,}

%
\author[3]{S.~Pingulkar,}

%
\author[3]{B.~Smithers,}
%
\author[3]{K.~Woodruff,}
%
\author[2]{C.~Adams,}
%
\author[22]{V.~\'Alvarez,}
%
\author[6]{L.~Arazi,}
%
\author[20]{I.J.~Arnquist,}
%
\author[4]{C.D.R~Azevedo,}
%
\author[2]{K.~Bailey,}
%
\author[22]{F.~Ballester,}
%
\author[19]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[14]{F.I.G.M.~Borges,}
%
\author[3]{N.~Byrnes,}
%
\author[19]{S.~C\'arcel,}
%
\author[19]{J.V.~Carri\'on,}
%
\author[23]{S.~Cebri\'an,}
%
\author[20]{E.~Church,}
%
\author[14]{C.A.N.~Conde,}
%
\author[11]{T.~Contreras,}
%
\author[21]{G.~D\'iaz,}
%
\author[19]{J.~D\'iaz,}
%
\author[5]{M.~Diesburg,}
%
\author[3]{R.~Dingler,}
%
\author[14]{J.~Escada,}
%
\author[22]{R.~Esteve,}
%
\author[6,19]{R.~Felkai,}
%
\author[13]{A.F.M.~Fernandes,}
%
\author[13]{L.M.P.~Fernandes,}
%
\author[16,9]{P.~Ferrario,}
%
\author[4]{A.L.~Ferreira,}
%
\author[13]{E.D.C.~Freitas,}
%
\author[16]{J.~Generowicz,}
%
\author[11]{S.~Ghosh,}
%
\author[8]{A.~Goldschmidt,}
%
\author[16,9,b]{J.J.~G\'omez-Cadenas,\note[b]{NEXT Co-spokesperson.}}
%
\author[21]{D.~Gonz\'alez-D\'iaz,}
%
\author[11]{R.~Guenette,}
%
\author[10]{R.M.~Guti\'errez,}
%
\author[11]{J.~Haefner,}
%
\author[2]{K.~Hafidi,}
%
\author[1]{J.~Hauptman,}
%
\author[13]{C.A.O.~Henriques,}
%
\author[21]{J.A.~Hernando~Morata,}
%
\author[16]{P.~Herrero,}
%
\author[22]{V.~Herrero,}
%
\author[6,7]{Y.~Ifergan,}
%
\author[2]{S.~Johnston,}
%
%\author[3]{B.J.P.~Jones,}
%
\author[19,21]{M.~Kekic,}
%
\author[18]{L.~Labarga,}
%
%\author[3]{A.~Laing,}
%
\author[5]{P.~Lebrun,}
%
\author[19]{N.~L\'opez-March,}
%
\author[10]{M.~Losada,}
%
\author[13]{R.D.P.~Mano,}
%
\author[11,8]{J.~Mart\'in-Albo,}
%
\author[19]{A.~Mart\'inez,}
%
\author[19,21,c]{G.~Mart\'inez-Lema,\note[c]{Now at Weizmann Institute of Science, Israel.}}
%
\author[3]{A.D.~McDonald,}
%
\author[16,9]{F.~Monrabal,}
%
\author[13]{C.M.B.~Monteiro,}
%
\author[22]{F.J.~Mora,}
%
\author[19]{J.~Mu\~noz~Vidal,}
%
\author[19]{P.~Novella,}
%
\author[3,b]{D.R.~Nygren,}
%
\author[19]{B.~Palmeiro,}
%
\author[5]{A.~Para,}
%
\author[12]{J.~P\'erez,}
%
\author[19]{M.~Querol,}
%
\author[6]{A.B.~Redwine,}
%
\author[21]{J.~Renner,}
%
\author[2]{J.~Repond,}
%
\author[2]{S.~Riordan,}
%
\author[17]{L.~Ripoll,}
%
\author[10]{Y.~Rodr\'iguez~Garc\'ia,}
%
\author[16]{J.~Rodr\'iguez,}
%
%\author[3]{L.~Rogers,}
%
\author[16,12]{B.~Romeo,}
%
\author[19]{C.~Romo-Luque,}
%
\author[14]{F.P.~Santos,}
%
\author[13]{J.M.F.~dos~Santos,}
%
\author[6]{A.~Sim\'on,}
%
\author[15,e]{C.~Sofka,\note[e]{Now at University of Texas at Austin, USA.}}
%
\author[19]{M.~Sorel,}
%
\author[15]{T.~Stiegler,}
%
\author[22]{J.F.~Toledo,}
%
\author[16]{J.~Torrent,}
%
\author[19]{A.~Us\'on,}
%
\author[4]{J.F.C.A.~Veloso,}
%
\author[15]{R.~Webb,}
%
\author[6,f]{R.~Weiss-Babai,\note[f]{On leave from Soreq Nuclear Research Center, Yavneh, Israel.}}
%
\author[15,g]{J.T.~White,\note[g]{Deceased.}}
%
%\author[3]{K.~Woodruff,}
%
\author[19]{N.~Yahlali}
%
\emailAdd{leslie.rogers@mavs.uta.edu}
%
\affiliation[1]{
Department of Physics and Astronomy, Iowa State University, 12 Physics Hall, Ames, IA 50011-3160, USA}
%
\affiliation[2]{
Argonne National Laboratory, Argonne, IL 60439, USA}
%
\affiliation[3]{
Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affiliation[4]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\affiliation[5]{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\affiliation[6]{
Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\affiliation[7]{
Nuclear Research Center Negev, Beer-Sheva, 84190, Israel}
%
\affiliation[8]{
Lawrence Berkeley National Laboratory (LBNL), 1 Cyclotron Road, Berkeley, CA 94720, USA}
%
\affiliation[9]{
Ikerbasque, Basque Foundation for Science, Bilbao, E-48013, Spain}
%
\affiliation[10]{
Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\affiliation[11]{
Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\affiliation[12]{
Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\affiliation[13]{
LIBPhys, Department of Physics, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\affiliation[14]{
LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\affiliation[15]{
Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\affiliation[16]{
Donostia International Physics Center (DIPC), Paseo Manuel Lardizabal, 4, Donostia-San Sebastian, E-20018, Spain}
%
\affiliation[17]{
Escola Polit\`ecnica Superior, Universitat de Girona, Av.~Montilivi, s/n, Girona, E-17071, Spain}
%
\affiliation[18]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Campus de Cantoblanco, Madrid, E-28049, Spain}
%
\affiliation[19]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\affiliation[20]{
Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\affiliation[21]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\affiliation[22]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\affiliation[23]{
Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA),Universidad de Zaragoza, Calle Pedro Cerbuna, 12, Zaragoza, E-50009, Spain}
%


==> Helium3 (2)/src/Commands.tex <==
\newcommand{\Ba}[1]{\ensuremath{^{#1}\mathrm{Ba}}\xspace}


%\newcommand{\Bi}[1]{\ensuremath{^{#1}\mathrm{Bi}}\xspace}
\newcommand{\Co}[1]{\ensuremath{^{#1}\mathrm{Co}}\xspace}
\newcommand{\Cs}[1]{\ensuremath{^{#1}\mathrm{Cs}}\xspace}
\newcommand{\K}[1]{\ensuremath{^{#1}\mathrm{K}}\xspace}
\newcommand{\Kr}[1]{\ensuremath{^{#1}\mathrm{Kr}}\xspace}
\newcommand{\Na}[1]{\ensuremath{^{#1}\mathrm{Na}}\xspace}
\newcommand{\Pb}[1]{\ensuremath{^{#1}\mathrm{Pb}}\xspace}
\newcommand{\Po}[1]{\ensuremath{^{#1}\mathrm{Po}}\xspace}
\newcommand{\Rb}[1]{\ensuremath{^{#1}\mathrm{Rb}}\xspace}
\newcommand{\Rn}[1]{\ensuremath{^{#1}\mathrm{Rn}}\xspace}
\newcommand{\Th}[1]{\ensuremath{^{#1}\mathrm{Th}}\xspace}
%\newcommand{\Tl}[1]{\ensuremath{^{#1}\mathrm{Tl}}\xspace}
\newcommand{\U}[1]{\ensuremath{^{#1}\mathrm{U}}\xspace}
%\newcommand{\Xe}[1]{\ensuremath{^{#1}\mathrm{Xe}}\xspace}
%\newcommand{\He}[1]{\ensuremath{^{#1}\mathrm{He}}\xspace}
\newcommand{\He}[1]{$^{#1}$He}
\newcommand{\Xe}[1]{$^{#1}$Xe}
\newcommand{\Bi}[1]{$^{#1}$Bi}
\newcommand{\Tl}[1]{$^{#1}$Tl}
\newcommand{\bbnonu}{$0\nu\beta\beta$}


\newcommand{\bbtwonu}{\ensuremath{2\nu\beta\beta}\xspace}
\newcommand{\bb}{\ensuremath{\beta\beta}\xspace}
\newcommand{\Qbb}{$Q_{\beta\beta}$}


\newcommand{\Qb}{$Q_{\beta}$}
\newcommand{\mbb}{\ensuremath{\langle m_{\nu} \rangle}}
\newcommand{\halflife}{\ensuremath{T_{1/2}}\xspace}  

\newcommand{\ckky}{keV$^{-1}$kg$^{-1}$yr$^{-1}$}


==> Helium3 (2)/src/ack.tex <==
The NEXT Collaboration acknowledges support from the following agencies and institutions: the European Research Council (ERC) under the Advanced Grant 339787-NEXT; the European Union’s Framework Programme for Research and Innovation Horizon 2020 (2014-2020) under the Marie Skłodowska-Curie Grant Agreements No. 674896, 690575 and 740055; the Ministerio de Econom\'ia y Competitividad and the Ministerio de Ciencia, Innovaci\'on y Universidades of Spain under grants FIS2014-53371-C04, RTI2018-095979, the Severo Ochoa Program SEV-2014-0398 and the Mar\'ia de Maetzu Program MDM-2016-0692; the GVA of Spain under grants PROMETEO/2016/120 and SEJI/2017/011; the Portuguese FCT under project PTDC/FIS-NUC/2525/2014, under project UID/FIS/04559/2013 to fund the activities of LIBPhys, and under grants PD/BD/105921/2014, SFRH/BPD/109180/2015 and SFRH/BPD/76842/2011; the U.S.\ Department of Energy under contracts number DE-AC02-06CH11357 (Argonne National Laboratory), DE-AC02-07CH11359 (Fermi National Accelerator Laboratory), DE-FG02-13ER42020 (Texas A\&M) and DE-SC0019223 / DE-SC0019054 (University of Texas at Arlington); and the University of Texas at Arlington. DGD acknowledges Ramon y Cajal program (Spain) under contract number RYC-2015-18820. We also warmly acknowledge the Laboratori Nazionali del Gran Sasso (LNGS) and the Dark Side collaboration for their help with TPB coating of various parts of the NEXT-White TPC. Finally, we are grateful to the Laboratorio Subterr\'aneo de Canfranc for hosting and supporting the NEXT experiment. 


==> src/ack.tex <==
The NEXT Collaboration acknowledges support from the following agencies and institutions: the European Research Council (ERC) under the Advanced Grant 339787-NEXT; the European Union’s Framework Programme for Research and Innovation Horizon 2020 (2014-2020) under the Marie Skłodowska-Curie Grant Agreements No. 674896, 690575 and 740055; the Ministerio de Econom\'ia y Competitividad and the Ministerio de Ciencia, Innovaci\'on y Universidades of Spain under grants FIS2014-53371-C04, RTI2018-095979, the Severo Ochoa Program SEV-2014-0398 and the Mar\'ia de Maetzu Program MDM-2016-0692; the GVA of Spain under grants PROMETEO/2016/120 and SEJI/2017/011; the Portuguese FCT under project PTDC/FIS-NUC/2525/2014, under project UID/FIS/04559/2013 to fund the activities of LIBPhys, and under grants PD/BD/105921/2014, SFRH/BPD/109180/2015 and SFRH/BPD/76842/2011; the U.S.\ Department of Energy under contracts number DE-AC02-06CH11357 (Argonne National Laboratory), DE-AC02-07CH11359 (Fermi National Accelerator Laboratory), DE-FG02-13ER42020 (Texas A\&M) and DE-SC0019223 / DE-SC0019054 (University of Texas at Arlington); and the University of Texas at Arlington. DGD acknowledges Ramon y Cajal program (Spain) under contract number RYC-2015-18820. We also warmly acknowledge the Laboratori Nazionali del Gran Sasso (LNGS) and the Dark Side collaboration for their help with TPB coating of various parts of the NEXT-White TPC. Finally, we are grateful to the Laboratorio Subterr\'aneo de Canfranc for hosting and supporting the NEXT experiment. 

